Writing your own book: A method for going from closed to open book QA to improve robustness and performance of smaller LLMs

We introduce two novel methods, Tree-Search and Self-contextualizing QA, designed to enhance the performance of large language models (LLMs) in question-answering tasks. Tree-Search is a sampling technique specifically created to extract diverse information from an LLM for a given prompt. Self-contextualizing QA leverages Tree-Search to enable the model to create its own context using a wide range of information relevant to the prompt, evaluate it explicitly and return a open book answer to the initial prompt . We demonstrate that the quality of generated answers improves according to various metrics, including accuracy, informativeness, coherence, and consistency, as evaluated by GPT3.5(text-davinci-003). Furthermore, we show that our methods result in increased robustness and that performance is positively correlated with tree size, benefiting both answer quality and robustness. Finally, we discuss other promising applications of Tree-Search, highlighting its potential to enhance a broad range of tasks beyond question-answering. \noindent We also discuss several areas for future work, including refining the Tree-Search and Self-Contextualizing QA methods, improving the coherence of the generated context, and investigating the impact of bootstrapping on model robustness

==> removed_text.tex <==
\end{enumerate}

\subsubsection{Future work}
While we have demonstrated the merits of Tree-Search as a novel decoding strategy, the current implementation in the paper is admittedly ad hoc, and there are several ways it can be improved, optimized, and expanded upon:

\begin{itemize}
\item \textbf{Optimizing high entropy identification:} High entropy positions are identified through two approaches: examining the odds of the top tokens and the number of remaining tokens given a probability cutoff. Multiple parameters can be optimized, including the odds ratio [R], the probability cutoff value [p], and the number of options given a cutoff [k(p)] that determine high entropy.

\item \textbf{Enhancing token selection:} The selection method for tokens in high entropy positions is limited to two ways in this paper: exhaustively choosing every token that meets the odds criteria or uniform random sampling in the position. To better steer the desired output and expand the applicability of Tree-Search to various NLP tasks, optimizing this feature is crucial.

\item \textbf{Exploring deeper searches:} We have exclusively used a depth of 3 in this paper, largely due to the computational limitations of the current implementation. Investigating the impact of deeper searches on the outcomes is an important area for future investigation, as it may reveal further potential for model steering and controllable exploration.

\item \textbf{Applying to other NLP tasks:} Building upon the merits of Tree-Search, future work may explore its application to other NLP tasks such as text summarization, machine translation, or creative text generation. Understanding how Tree-Search can be adapted and optimized for these tasks would provide valuable insights into its broader potential.

\item \textbf{Model interpretability and uncertainty quantification:} By analyzing high entropy positions and the distribution of token probabilities, Tree-Search can offer valuable insights into the model's uncertainty. Future research could focus on leveraging these insights to improve model performance, develop more robust strategies for extracting information, and enhance model interpretability.

\item \textbf{Hallucinations:} Tree-Search also offers a valuable opportunity to study hallucinations in large language models, which refers to instances where the model generates incorrect facts or statements. Given the nature of LLMs, it is inevitable that some of the various outputs produced in response to a question will be false or misleading. By systematically examining these incorrect outputs, researchers can gain insights into the factors that contribute to hallucinations in the model.

By analyzing the different ways in which questions are answered, it may be possible to identify specific phrasings, types of words (e.g., certain nouns, prepositions, or verbs), or other linguistic patterns that are more likely to lead the model to produce incorrect answers. Understanding these patterns could help quantify the likelihood of the model hallucinating and inform targeted interventions to improve the model's performance.

For instance, researchers could develop techniques to filter out or eliminate specific words and sentences that are more likely to trigger hallucinations, thereby mitigating the risks associated with the model's outputs. Alternatively, this information could be used to fine-tune the model, refining its knowledge and reducing its propensity for generating incorrect responses.


\item \textbf{Insights into Model Uncertainty and Explainability:} Tree-Search presents a unique opportunity to delve into model uncertainty and enhance the explainability of large language models. By scrutinizing high entropy positions and the distribution of token probabilities, it uncovers valuable insights into areas of uncertainty within the model, which can be instrumental in designing interventions for performance improvement or robust information extraction strategies.

Moreover, Tree-Search's ability to generate a myriad of facts or rephrasings for a given question offers a lens into how the model distributes and represents information. This, in conjunction with a method suggested by Meng et al.~\cite{Meng2022}, which identifies specific fact locations within a model, can illuminate the underlying structure of the model's knowledge representation and its interconnections between related facts and concepts.

Such an approach could aid in identifying redundancies and inconsistencies in the model's knowledge storage, leading to potential enhancements in performance and efficiency. Ultimately, this could contribute significantly to developing more interpretable, transparent AI systems—a critical step for fostering trust and ensuring ethical deployment of AI technologies across various domains.
\subsubsection{Future Work: Closed to open book QA}\label{sec:future_qa}
In this paper, we employed a simplistic approach for assembling the context. The only processing performed on the tree is the removal of duplicated text, maintaining the tree structure as shown in figure~\ref{fig:tree}. While this results in somewhat incoherent text (though surprisingly coherent in some cases), as demonstrated in the Results section, it still contributes to improved performance. Since the model is trained to understand coherent texts, it is reasonable to assume that providing more coherent and higher-quality context would further enhance the results. We propose several avenues for future work to build upon and improve the closed to open book Q\&A approach.

\noindent One potential direction is enhancing context coherence. Future work may focus on refining the process of context construction, training the model to better identify and correct errors in the context, and developing mechanisms for assessing the reliability of the extracted information. Two primary methods for improving the text are proposed: first, training the model itself to convert the incoherent output into coherent output; and second, attaching a separate model to process the text and generate coherent context for the model to use when re-prompting it.

\noindent Another area for exploration is optimizing context selection. Instead of solely relying on Tree-Search outputs, alternative context selection methods could be investigated, such as using similarity metrics or external knowledge sources to rank and filter the extracted information. This may help create higher-quality and more relevant context for the model to use when re-prompting it.

\noindent Furthermore, an iterative approach to context refinement could be explored, where the model is prompted multiple times, each time with an improved context generated by the previous iteration. This bootstrapping process could lead to more accurate and coherent context generation over time.

\noindent Finally, investigating the applicability of the closed to open book Q\&A approach to other tasks or domains, such as medical or legal, would provide valuable insights into its broader potential and the necessary adaptations for optimal performance in these specialized areas.
